DreamDDP: Accelerating Data Parallel Distributed LLM Training with Layer-wise Scheduled Partial Synchronization

The growth of large language models (LLMs) increases challenges of accelerating distributed training across multiple GPUs in different data centers. Moreover, concerns about data privacy and data exhaustion have heightened interest in geo-distributed data centers. Communication in geo-distributed data parallel training (DDP) with stochastic gradient descent (S-SGD) is the main bottleneck in low-bandwidth environments. Local SGD mitigates communication overhead by reducing synchronization frequency, and recent studies have successfully applied it to geo-distributedly pre-train LLMs. However, we identify that its model synchronization mechanism prevents overlapping communication and computation, which makes the system lose opportunities to overlap communication and computation. To overcome this limitation, we expand the design space of local SGD by layer-wisely decoupling model synchronization. In each iteration, only some layers are synchronized instead of the entire model after a specific number of iterations. Leveraging this methodology, we introduce DreamDDP, a training framework to accelerate low-bandwidth distributed training with three key innovations: (1) partial local SGD with theoretical assurances of convergence rates comparable to S-SGD; (2) overlapping parameter synchronization with computation without extra GPU memory occupation; (3) identifying and exploiting three properties to schedule the communication and computation to reduce the training time based on fine-grained profiling of layer-wise communication and computation time. Empirical evaluations conducted on 32 GPUs using prominent deep learning models, including ResNet-18, ResNet-50, GPT-2, and Llama-2, demonstrate that DreamDDP enhances the convergence properties of Local SGD (and Adam) and achieves speedups ranging from $1.49\times$ to $3.91\times$ over leading baseline methods.

==> origin_proof.tex <==
\begin{proof}[Proof of Lemma~\ref{lemma:b1}]
Using the update Eq.~\ref{eq:partial-LSGD}, we have 
\begin{equation}
\small
\label{eq:b0}
\begin{split}
||\Bar{w}_{r+1}-w^*||^2=&||\Bar{w}_r-\eta_rg_r-w^*-\eta_r\Bar{g}_r+\eta_r\Bar{g}_r||^2\\
    =&||\Bar{w}_r-\eta_r\Bar{g}_r-w^*||^2+\eta_r^2||g_r-\Bar{g}_r||^2\\
    &+2\eta_r\langle\Bar{w}_r-w^*-\eta_r\Bar{g}_r,g_r-\Bar{g}_r\rangle.
\end{split}
\end{equation}
By $L$-smoothness and $\mu$-strong convexity of $f$, the first term is bounded as 
\begin{equation}
\small
\label{eq:b1}
\begin{split}
    &||\Bar{w}_r-\eta_r\Bar{g}_r-w^*||^2=||\Bar{w}_r-w^*||^2+\eta_r^2||\Bar{g}_r||^2-2\langle\Bar{w}_r-w^*,\eta_r\Bar{g}_r\rangle\\
    &\leq ||\Bar{w}_r-w^*||^2+\eta_r^2\frac{1}{M}\sum_{k=1}^K||\nabla f(w_r^k)||^2\\
    &-\frac{2\eta_r}{M}\sum_{k=1}^K\langle\Bar{w}_r-w^k_r+w^k_r-w^*,\nabla f(w_r^k)\rangle\\
    &=||\Bar{w}_r-w^*||^2+\eta_r^2\frac{1}{M}\sum_{k=1}^K||\nabla f(w_r^k)-\nabla f(w^*)||^2\\
    &-\frac{2\eta_r}{M}\sum_{k=1}^K\langle w^k_r-w^*,\nabla f(w_r^k)\rangle-\frac{2\eta_r}{M}\sum_{k=1}^K\langle\Bar{w}_r-w^k_r,\nabla f(w_r^k)\rangle\\
\end{split}
\end{equation}
By $L$-smoothness,
\begin{equation}
\small
    ||\nabla f(w_r^k)-\nabla f(w^*)||^2\leq2L(f(w_r^k)-f^*)
\end{equation}
By $\mu$-strong convexity
\begin{equation}
\small
    -\langle w_r^k-w^*,\nabla f(w_r^k)\rangle\leq-(f(w_r^k)-f^*)-\frac{\mu}{2}||w_r^k-w^*||^2
\end{equation}
To estimate the last term in (\ref{eq:b1}), we use $2\langle a,b\rangle\leq\gamma||a||^2+\gamma^{-1}||b||^2$ for $\gamma>0$,
\begin{equation}
\small
\label{eq:b2}
\begin{split}
    &-2\langle\Bar{w}_t-w_r^k,\nabla f(w_r^k)\rangle\leq2L||\Bar{w}_r-w_r^k||^2+\frac{1}{2L}||\nabla f(w_r^k)||^2\\
    &=2L||\Bar{w}_r-w_r^k||^2+\frac{1}{2L}||\nabla f(w_r^k)-\nabla f(w^*)||^2\\
    &\leq2L||\Bar{w}_r-w_r^k||^2+(f(w_r^k)-f^*)
\end{split}
\end{equation}
By applying these estimates to (\ref{eq:b1}) we get
\begin{equation}
\small
\label{eq:b3}
    \begin{split}
        &||\Bar{w}_r-w^*-\eta_r\Bar{g}_r||^2\leq||\Bar{w}_r-w^*||^2+\frac{2\eta_rL}{M}\sum_{k=1}^K||\Bar{w}_r-w_r^k||^2\\
        &+\frac{2\eta_r}{M}\sum_{k=1}^K((\eta_rL-\frac{1}{2})(f(w_r^k)-f^*)-\frac{\mu}{2}||w_r^k-w^*||^2)
    \end{split}
\end{equation}
For $\eta_r\leq \frac{1}{4L}$ it holds $(\eta_rL-\frac{1}{2})\leq -\frac{1}{4}$. By convexity of $a(f(w)-f^*)+b||w-w^*||^2$ for $a,b\geq0$,
\begin{equation}
\small
    \begin{split}
        &-\frac{1}{M}\sum_{k=1}^K(a(f(w_r^k)-f^*)+b||w_r^k-w^*||^2)\\
        &\leq-(a(f(\Bar{w}_r)-f^*)+b||\Bar{w}_r-w^*||^2).
    \end{split}
\end{equation}
Hence, we can continue in (\ref{eq:b3}) and obtain
\begin{equation}
\small
\label{eq:b4}
    \begin{split}
        &||\Bar{w}_r-w^*-\eta_r\Bar{g}_r||^2\leq(1-\mu\eta_r)||\Bar{w}_r-w^*||^2\\
        &-\frac{1}{2}\eta_r(f(\Bar{w}_r)-f^*)+\frac{2\eta_rL}{M}\sum_{k=1}^K||\Bar{w}_r-w_r^k||^2
    \end{split}
\end{equation}
Finally, we can plug (\ref{eq:b4}) back into (\ref{eq:b0}). By taking expectation we get 
\begin{equation}
\label{eq:b5}
\small
\begin{split}
    &\mathbb{E}||\Bar{w}_{r+1}-w^*||^2\\
    \leq&(1-\mu\eta_r)\mathbb{E}||\Bar{w}_r-w^*||^2+\eta_r^2\mathbb{E}||g_r-\Bar{g}_r||^2\\
    &-\frac{1}{2}\eta_r\mathbb{E}(f(\Bar{w}_r)-f^*)+\frac{2L\eta_r }{M}\sum_{k=1}^K\mathbb{E}||\Bar{w}_r-w_{r}^{k}||^2
\end{split}
\end{equation}
\end{proof}











